Classical Stability Margins by PID Control

Proportional-Integral-Derivative (PID) control has been the workhorse of control technology for about a century. Yet to this day, designing and tuning PID controllers relies mostly on either tabulated rules (Ziegler-Nichols) or on classical graphical techniques (Bode). Our goal in this paper is to take a fresh look on PID control in the context of optimizing stability margins for low-order (first- and second-order) linear time-invariant systems. Specifically, we seek to derive explicit expressions for gain and phase margins that are achievable using PID control, and thereby gain insights on the role of unstable poles and nonminimum-phase zeros in attaining robust stability. In particular, stability margins attained by PID control for minimum-phase systems match those obtained by more general control, while for nonminimum-phase systems, PID control achieves margins that are no worse than those of general control modulo a predetermined factor. Furthermore, integral action does not contribute to robust stabilization beyond what can be achieved by PD control alone.

==> myieeebibfile.tex <==
@article{makila1998comments,
  title={Comments on ``Robust, fragile, or optimal?"[with reply]},
  author={Makila, Pertti M},
  journal={IEEE Transactions on Automatic Control},
  volume={43},
  number={9},
  pages={1265--1268},
  year={1998},
  publisher={IEEE}
}

@article{zames1981feedback,
  title={Feedback and optimal sensitivity: Model reference transformations, multiplicative seminorms, and approximate inverses},
  author={Zames, George},
  journal={IEEE Transactions on Automatic Control},
  volume={26},
  number={2},
  pages={301--320},
  year={1981},
  publisher={IEEE}
}

@article{doyle1978guaranteed,
  title={Guaranteed margins for {L}{Q}{G} regulators},
  author={Doyle, John C},
  journal={IEEE Transactions on Automatic Control},
  volume={23},
  number={4},
  pages={756--757},
  year={1978},
  publisher={IEEE}
}


@article{ziegler1942optimum,
  title={Optimum settings for automatic controllers},
  author={Ziegler, John G and Nichols, Nathaniel B and Rochester, N Y},
  journal={Trans. ASME},
  volume={64},
  number={11},
  pages={759--765},
  year={1942}
}


@article{tannenbaum1982modified,
  title={Modified Nevanlinna-Pick interpolation and feedback stabilization of linear plants with uncertainty in the gain factor},
  author={Tannenbaum, Allen},
  journal={International Journal of Control},
  volume={36},
  number={2},
  pages={331--336},
  year={1982},
  publisher={Taylor \& Francis}
}

@inproceedings{mao2021maximal,
  title={Maximal Gain and Phase Margins Attainable by {P}{I}{D} Control},
  author={Mao, Qi  and Xu, Yong and Chen,  Jianqi  and Chen, Jie and  Georgiou, Tryphon},
  booktitle={2021 60th IEEE Conference on Decision and Control (CDC)},
  pages={1820--1825},
  address={Austin, Texas},
  month={December},
  year={2021},
  organization={IEEE}
}

%%%%[1]
@inproceedings{cockburn1992constructive,
  title={A constructive solution to the gain-phase margin problem},
  author={Cockburn, Juan C and Sidar, Yariv and Tannenbaum, Allen},
  booktitle={[1992] Proceedings of the 31st IEEE Conference on Decision and Control},
  pages={682--683},
  address={Tucson, AZ},
  month={December},
  year={1992},
  organization={IEEE}
}

%%%%[2]
@article{safonov1977gain,
  title={Gain and phase margin for multiloop {L}{Q}{G} regulators},
  author={Safonov, Michael and Athans, Michael},
  journal={IEEE Transactions on Automatic Control},
  volume={22},
  number={2},
  pages={173--179},
  year={1977},
  publisher={IEEE}
}

%%%%[3]
@article{tannenbaum1986multivariable,
  title={On the multivariable gain margin problem},
  author={Tannenbaum, Allen},
  journal={Automatica},
  volume={22},
  number={3},
  pages={381--383},
  year={1986},
  publisher={Elsevier}
}

@book{Ball90,
  title={Interpolation of Rational Matrix Functions},
  author={Ball, Joseph and Gohberg, Israel and Rodman, Leiba},
  year={1990},
 publisher={Birkhauser}
}

@book{Bode45,
  title={Network Analysis and Feedback Amplifier Design},
  author={Bode, H.W.},
  year={1945},
  address={},
  publisher={Van Nostrand}
}

@book{Horowitz63,
  title={Synthesis of Feedback systems},
  author={I. M. Horowitz},
  year={1963},
  publisher={Academic Press},
}

@book{tannenbaum1981invariance,
  title={Invariance and System Theory: Algebraic and Geometric Aspects},
  author={Tannenbaum, Allen},
  year={1981},
  address={London},
  publisher={Springer}
}

%%%%[4]
@article{feintuch1986gain,
  title={Gain optimization for distributed plants},
  author={Feintuch, Avraham and Tannenbaum, Allen},
  journal={Systems \& Control Letters},
  volume={6},
  number={5},
  pages={295--301},
  year={1986},
  publisher={Elsevier}
}

%%%%[5]
@inproceedings{tantaris2003gain,
  title={Gain/phase margin design with first order controllers},
  author={Tantaris, RN and Keel, LH and Bhattacharyya, SP},
  booktitle={Proceedings of the 2003 American Control Conference},
  volume={5},
  pages={3937--3942},
  address={Denver, CO},
  month={June},
  year={2003},
  organization={IEEE}
}

%%%%[6]
@article{cockburn1995stability,
  title={Stability margin optimization via interpolation and conformal mappings},
  author={Cockburn, Juan C and Sidar, Yariv and Tannenbaum, Allen R},
  journal={IEEE Transactions on Automatic Control},
  volume={40},
  number={6},
  pages={1066--1070},
  year={1995},
  publisher={IEEE}
}

@article{olbrot1994robust,
  title={Robust stabilization: Some extensions of the gain margin maximization problem},
  author={Olbrot, AW and Nikodem, M},
  journal={IEEE Transactions on Automatic Control},
  volume={39},
  number={3},
  pages={652--657},
  year={1994},
  publisher={IEEE}
}

%%%%[7]
@article{ho1996performance,
  title={Performance and gain and phase margins of well-known {P}{I}{D} tuning formulas},
  author={Ho, Weng Khuen and Gan, OP and Tay, Ee Beng and Ang, EL},
  journal={IEEE Transactions on Control Systems Technology},
  volume={4},
  number={4},
  pages={473--477},
  year={1996},
  publisher={IEEE}
}

%%%%[8]
@article{paraskevopoulos2006pid,
  title={{P}{I}{D}-type controller tuning for unstable first order plus dead time processes based on gain and phase margin specifications},
  author={Paraskevopoulos, Paraskevas N and Pasgianos, George D and Arvanitis, Konstantinos G},
  journal={IEEE Transactions on Control Systems Technology},
  volume={14},
  number={5},
  pages={926--936},
  year={2006},
  publisher={IEEE}
}

%%%%
@article{maeda1986infinite,
  title={Infinite gain margin problem in multivariable feedback systems},
  author={Maeda, H and Vidyasagar, M},
  journal={Automatica},
  volume={22},
  number={1},
  pages={131--133},
  year={1986},
  publisher={Elsevier}
}

%%%%
@inproceedings{yan1989simultaneous,
  title={The simultaneous optimization problem for sensitivity and gain margin},
  author={Yan, Weiyong and Anderson, Brian DO},
  booktitle={Proceedings of the 28th IEEE Conference on Decision and Control},
  pages={1697--1702},
  address={Tampa, FL},
  month={December},
  year={1989},
  organization={IEEE}
}

%%%%[9]
@article{wang2009synthesis,
  title={Synthesis of phase-lead/lag compensators with complete information on gain and phase margins},
  author={Wang, De-Jin},
  journal={Automatica},
  volume={45},
  number={4},
  pages={1026--1031},
  year={2009},
  publisher={Elsevier}
}

%%%%[10]
@article{kalman1964linear,
  title={When is a linear control system optimal?},
  author={Kalman, Rudolf Emil},
  journal={Trans ASME, J. Basic Eng.},
  volume={86},
  number={1},
  pages={51--60},
  year={1964}
}

%%%%[11]
@article{willems1978return,
  title={The return difference for discrete-time optimal feedback systems},
  author={Willems, Jacques L and van de Voorde, Herman},
  journal={Automatica},
  volume={14},
  number={5},
  pages={511--513},
  year={1978},
  publisher={Elsevier}
}

%%%%[12]
@article{tannenbaum1980feedback,
  title={Feedback stabilization of linear dynamical plants with uncertainty in the gain factor},
  author={Tannenbaum, Allen},
  journal={International Journal of Control},
  volume={32},
  number={1},
  pages={1--16},
  year={1980},
  publisher={Taylor $\&$ Francis}
}

%%%%[13]
@article{lee1987vibrational,
  title={Vibrational feedback control: Zeros placement capabilities},
  author={Lee, Soodong and Meerkov, SEMYONM and Runolfsson, Thordur},
  journal={IEEE Transactions on Automatic Control},
  volume={32},
  number={7},
  pages={604--611},
  year={1987},
  publisher={IEEE}
}


%%%%[14]
@article{francis1988stability,
  title={Stability theory for linear time-invariant plants with periodic digital controllers},
  author={Francis, Bruce A and Georgiou, Tryphon T},
  journal={IEEE Transactions on Automatic Control},
  volume={33},
  number={9},
  pages={820--832},
  year={1988},
  publisher={IEEE}
}

%%%%[15]
@article{samad2017survey,
  title={A survey on industry impact and challenges thereof [technical activities]},
  author={Samad, Tariq},
  journal={IEEE Control Systems Magazine},
  volume={37},
  number={1},
  pages={17--18},
  year={2017},
  publisher={IEEE}
}

%%%%[16]
@article{ho1995tuning,
  title={Tuning of {P}{I}{D} controllers based on gain and phase margin specifications},
  author={Ho, Weng Khuen and Hang, Chang Chieh and Cao, Lisheng S},
  journal={Automatica},
  volume={31},
  number={3},
  pages={497--502},
  year={1995},
  publisher={Elsevier}
}


%%%%[]
@article{khargonekar1985non,
  title={Non-{E}uclidian metrics and the robust stabilization of systems with parameter uncertainty},
  author={Khargonekar, Pramod and Tannenbaum, Allen},
  journal={IEEE Transactions on Automatic Control},
  volume={30},
  number={10},
  pages={1005--1013},
  year={1985},
  publisher={IEEE}
}

%%%%[]
@book{doyle2013feedback,
  title={Feedback Control Theory},
  author={Doyle, John C and Francis, Bruce A and Tannenbaum, Allen R},
  year={2013},
  publisher={Courier Corporation}
}

%%%%[]
@article{frank1946zeros,
  title={On the zeros of polynomials with complex coefficients},
  author={Frank, Evelyn},
  journal={Bulletin of the American Mathematical Society},
  volume={52},
  number={2},
  pages={144--157},
  year={1946}
}

%%%%[]
@book{li2010introduction,
  title={Introduction to Feedback Control},
  author={Li, Qiu},
  year={2010},
  publisher={Pearson Education India}
}

%%%%[]
@article{Silva2002New,
  title={New results on the synthesis of {P}{I}{D} controllers},
  author={Silva, Guillermo J. and Datta, Aniruddha and Bhattacharyya, S. P.},
  journal={IEEE Transactions on Automatic Control},
  volume={47},
  number={2},
  pages={241-252},
  year={2002},
}

%%%%[]
@article{ma2018delay,
  title={Delay margin of low-order systems achievable by {P}{I}{D} controllers},
  author={Ma, Dan and Chen, Jie},
  journal={IEEE Transactions on Automatic Control},
  volume={64},
  number={5},
  pages={1958--1973},
  year={2018},
  publisher={IEEE}
}


%%%%[]
@article{ho1998optimal,
  title={Optimal gain and phase margin tuning for {P}{I}{D} controllers},
  author={Ho, Weng Khuen and Lim, Khiang Wee and Xu, Wen},
  journal={Automatica},
  volume={34},
  number={8},
  pages={1009--1014},
  year={1998},
  publisher={Elsevier}
}

%%%%[]
@article{ho1993tuning,
  title={Tuning of {P}{I}{D} controllers based on gain and phase margin specifications},
  author={Ho, WK and Hang, CC and Cao, LS},
  journal={IFAC Proceedings Volumes},
  volume={26},
  number={2},
  pages={199--202},
  year={1993},
  publisher={Elsevier}
}

%%%%[]
@article{ho1999getting,
  title={Getting more phase margin and performance out of {P}{I}{D} controllers},
  author={Ho, Weng Khuen and Lim, Khiang Wee and Hang, Chang Chieh and Ni, LY},
  journal={Automatica},
  volume={35},
  number={9},
  pages={1579--1585},
  year={1999},
  publisher={Elsevier}
}

%%%%[]
@article{rotstein1991simple,
  title={Simple {P}{I} and {P}{I}{D} tuning for open-loop unstable systems},
  author={Rotstein, Guillermo E and Lewin, Daniel R},
  journal={Industrial \& Engineering Chemistry Research},
  volume={30},
  number={8},
  pages={1864--1869},
  year={1991},
  publisher={ACS Publications}
}

%%%%[]
@article{ho1997self,
  title={Self-tuning {P}{I}{D} control of a plant with under-damped response with specifications on gain and phase margins},
  author={Ho, Weng Khuen and Hang, Chang Chieh and Zhou, Junhong},
  journal={IEEE Transactions on Control Systems Technology},
  volume={5},
  number={4},
  pages={446--452},
  year={1997},
  publisher={IEEE}
}

%%%%[]
@article{park1998enhanced,
  title={An enhanced {P}{I}{D} control strategy for unstable processes},
  author={Park, Jin Hyun and Sung, Su Whan and Lee, In-Beum},
  journal={Automatica},
  volume={34},
  number={6},
  pages={751--756},
  year={1998},
  publisher={Elsevier}
}

%%%%[]
@article{paraskevopoulos2004new,
  title={New tuning and identification methods for unstable first order plus dead-time processes based on pseudoderivative feedback control},
  author={Paraskevopoulos, Paraskevas N and Pasgianos, George D and Arvanitis, Konstantinos G},
  journal={IEEE transactions on control systems technology},
  volume={12},
  number={3},
  pages={455--464},
  year={2004},
  publisher={IEEE}
}

%%%%[]
@article{aastrom2004revisiting,
  title={Revisiting the Ziegler--Nichols step response method for {P}{I}{D} control},
  author={{\AA}str{\"o}m, Karl Johan and H{\"a}gglund, Tore},
  journal={Journal of Process Control},
  volume={14},
  number={6},
  pages={635--650},
  year={2004},
  publisher={Elsevier}
}

%%%%[]
@article{yaniv2004design,
  title={Design of {P}{I}{D} controllers satisfying gain margin and sensitivity constraints on a set of plants},
  author={Yaniv, Oded and Nagurka, M},
  journal={Automatica},
  volume={40},
  number={1},
  pages={111--116},
  year={2004},
  publisher={Elsevier}
}

%%%%[]
@article{krstic2017applicability,
  title={On the applicability of {P}{I}{D} control to nonlinear second-order systems},
  author={Krstic, Miroslav},
  journal={National Science Review},
  volume={4},
  number={5},
  pages={668--668},
  year={2017},
  publisher={Oxford University Press}
}

%%%%[]
@book{aastrom1995pid,
  title={{P}{I}{D} Controllers: Theory, Design, and Tuning},
  author={{\AA}str{\"o}m, Karl Johan and H{\"a}gglund, Tore},
  volume={2},
  year={1995},
  publisher={Instrument Society of America, Research Triangle Park, NC}
}


%%%%[]
@article{el1985gap,
  title={The gap metric: Robustness of stabilization of feedback systems},
  author={El-Sakkary, Ahmed},
  journal={IEEE Transactions on Automatic Control},
  volume={30},
  number={3},
  pages={240--247},
  year={1985},
  publisher={IEEE}
}

%%%%[]
@article{zames1981unstable,
  title={Unstable systems and feedback: The gap metric},
  author={Zames, George},
  journal={IFAC Proceedings Volumes},
  volume={14},
  number={2},
  pages={149-152},
  year={1981},
  publisher={Elsevier}
}

%%%%[]
@inproceedings{georgiou1989optimal,
  title={Optimal robustness in the gap metric},
  author={Georgiou, Tryphon T and Smith, Malcolm C},
  booktitle={Proceedings of the 28th IEEE Conference on Decision and Control,},
  pages={2331--2336},
  address={Tampa, FL},
  month={December},
  year={1989},
  organization={IEEE}
}

%%%%[]
@article{vidyasagar1984graph,
  title={The graph metric for unstable plants and robustness estimates for feedback stability},
  author={Vidyasagar, Mathukumalli},
  journal={IEEE Transactions on Automatic Control},
  volume={29},
  number={5},
  pages={403--418},
  year={1984},
  publisher={IEEE}
}

%%%%[]
@article{georgiou1988computation,
  title={On the computation of the gap metric},
  author={Georgiou, Tryphon T},
  journal={Systems \& Control Letters},
  volume={11},
  number={4},
  pages={253--257},
  year={1988},
  publisher={Elsevier}
}

%%%%[]
@inproceedings{georgiou1990robust,
  title={Robust stabilization in the gap metric: Controller design for distributed plants},
  author={Georgiou, Tryphon T and Smith, Malcolm C},
  booktitle={1990 American Control Conference},
  pages={1570--1575},
  address={San Diego, CA},
  month={May},
  year={1990},
  organization={IEEE}
}

%%%%[]
@article{vinnicombe1993frequency,
  title={Frequency domain uncertainty and the graph topology},
  author={Vinnicombe, Glenn},
  journal={IEEE Transactions on Automatic Control},
  volume={38},
  number={9},
  pages={1371--1383},
  year={1993},
  publisher={IEEE}
}

%%%%[]
@book{zhou1996robust,
  title={Robust and Optimal Control},
  author={Zhou, Kemin and Doyle, John Comstock and Glover, Keith and others},
  volume={40},
  year={1996},
  publisher={Prentice Hall New Jersey}
}

%%%%[]
@article{francis1987linear,
  title={Linear Control Theory with an ${{{\rm{H}}}_\infty }$ Optimality Criterion},
  author={Francis, Bruce A and Doyle, John C},
  journal={SIAM Journal on Control and Optimization},
  volume={25},
  number={4},
  pages={815--844},
  year={1987},
  publisher={SIAM}
}

%%%%[]
@inproceedings{cusumano1988nonlinear,
  title={Nonlinear feedback vs. linear feedback for robust stabilization},
  author={Cusumano, Salvatore J and Poolla, Kameshwar},
  booktitle={Proceedings of the 27th IEEE Conference on Decision and Control},
  pages={1776--1780},
  address={Austin, TX},
  month={December},
  year={1988},
  organization={IEEE}
}

%%%%[]
@article{gundecs2020controller,
  title={Controller redesign for delay margin improvement},
  author={G{\"u}nde{\c{s}}, A Nazli and {\"O}zbay, Hitay},
  journal={Automatica},
  volume={113},
  pages={108790},
  year={2020},
  publisher={Elsevier}
}


%%%%[]
@article{michiels2002continuous,
  title={Continuous pole placement for delay equations},
  author={Michiels, Wim and Engelborghs, Koen and Vansevenant, Patrick and Roose, Dirk},
  journal={Automatica},
  volume={38},
  number={5},
  pages={747--761},
  year={2002},
  publisher={Elsevier}
}


%%%%[]
@article{zitek2013dimensional,
  title={Dimensional analysis approach to dominant three-pole placement in delayed {P}{I}{D} control loops},
  author={Z{\'\i}tek, Pavel and Fi{\v{s}}er, Jarom{\'\i}r and Vyhl{\'\i}dal, Tom{\'a}{\v{s}}},
  journal={Journal of Process Control},
  volume={23},
  number={8},
  pages={1063--1074},
  year={2013},
  publisher={Elsevier}
}

%%%%[]
@article{wang2017new,
  title={New results on {P}{I}{D} controller design of discrete-time systems via pole placement},
  author={Wang, Honghai and Liu, Jianchang and Yu, Xia and Tan, Shubin and Zhang, Yu},
  journal={IFAC-PapersOnLine},
  volume={50},
  number={1},
  pages={6703--6708},
  year={2017},
  publisher={Elsevier}
}

%%%%[]
@article{zhao2017capability,
  title={On the capability of {P}{I}{D} control for nonlinear uncertain systems},
  author={Zhao, Cheng and Guo, Lei},
  journal={IFAC-PapersOnLine},
  volume={50},
  number={1},
  pages={1521--1526},
  year={2017},
  publisher={Elsevier}
}

%%%%[]
@article{zhao2020control,
  title={Control of Nonlinear Uncertain Systems by Extended {P}{I}{D}},
  author={Zhao, Cheng and Guo, Lei},
  journal={IEEE Transactions on Automatic Control},
  volume={66},
  number={8},
  pages={ 3840--3847},
  year={2020},
  publisher={IEEE}
}

%%%%[]
@article{zhang2019theory,
  title={Theory and design of {P}{I}{D} controller for nonlinear uncertain systems},
  author={Zhang, Jinke and Guo, Lei},
  journal={IEEE Control Systems Letters},
  volume={3},
  number={3},
  pages={643--648},
  year={2019},
  publisher={IEEE}
}

%%%%[]
@book{marden1949geometry,
  title={Geometry of Polynomials},
  author={Marden, Morris},
  year={1949},
  publisher={American Mathematical Soc.}
}

%%%%[]
@article{chen2000logarithmic,
  title={Logarithmic integrals, interpolation bounds, and performance limitations in {M}{I}{M}{O} feedback systems},
  author={Chen, Jie},
  journal={IEEE Transactions on Automatic Control},
  volume={45},
  number={6},
  pages={1098--1115},
  year={2000},
  publisher={IEEE}
}


%%%%[]
@article{chen2021delay,
  title={Delay Robustness of {P}{I}{D} Control of Second-Order Systems: Pseudo-Concavity, Exact Delay Margin, and Performance Trade-Off},
  author={Chen, Jianqi and Ma, Dan and Xu, Yong and Chen, Jie},
  journal={IEEE Transactions on Automatic Control},
  volume={67},
  number={3},
  pages={1194--1209},
  year={2021},
  publisher={IEEE}
}

%%%%[]
@book{aastrom2006advanced,
  title={Advanced {P}{I}{D} control},
  author={{\AA}str{\"o}m, Karl Johan and H{\"a}gglund, Tore and Astrom, Karl J},
  volume={461},
  year={2006},
  publisher={ISA-The Instrumentation, Systems, and Automation Society Research Triangle Park}
}

%%%%[]
@article{garpinger2014performance,
  title={Performance and robustness trade-offs in {P}{I}{D} control},
  author={Garpinger, Olof and H{\"a}gglund, Tore and {\AA}str{\"o}m, Karl Johan},
  journal={Journal of Process Control},
  volume={24},
  number={5},
  pages={568--577},
  year={2014},
  publisher={Elsevier}
}

%%%%[]
@article{apostol1970resultants,
  title={Resultants of cyclotomic polynomials},
  author={Apostol, Tom M},
  journal={Proceedings of the American Mathematical Society},
  volume={24},
  number={3},
  pages={457--462},
  year={1970}
}

%%%%[]
@article{anderson1998descartes,
  title={Descartes' rule of signs revisited},
  author={Anderson, Bruce and Jackson, Jeffrey and Sitharam, Meera},
  journal={The American Mathematical Monthly},
  volume={105},
  number={5},
  pages={447--451},
  year={1998},
  publisher={Taylor \& Francis}
}

%%%%[]
@book{borwein1995polynomials,
  title={Polynomials and Polynomial Inequalities},
  author={Borwein, Peter and Erd{\'e}lyi, Tam{\'a}s},
  volume={161},
  year={1995},
  publisher={Springer Science \& Business Media}
}

%%%%[]
@article{boros2005sums,
  title={Sums of arctangents and some formulas of Ramanujan},
  author={Boros, George and Moll, Victor H},
  journal={SCIENTIA Series A: Mathematical Sciences},
  volume={10},
  pages={13--24},
  year={2005}
}

%%%%[]
@article{chen2017stability,
  title={Stability analysis of polynomially dependent systems by eigenvalue perturbation},
  author={Chen, Jie and Fu, Peilin and M{\'e}ndez-Barrios, C{\'e}sar-Fernando and Niculescu, Silviu-Iulian and Zhang, Hongwei},
  journal={IEEE Transactions on Automatic Control},
  volume={62},
  number={11},
  pages={5915--5922},
  year={2017},
  publisher={IEEE}
}

